Chameleon: Fast-slow Neuro-symbolic Lane Topology Extraction

Lane topology extraction involves detecting lanes and traffic elements and determining their relationships, a key perception task for mapless autonomous driving. This task requires complex reasoning, such as determining whether it is possible to turn left into a specific lane. To address this challenge, we introduce neuro-symbolic methods powered by vision-language foundation models (VLMs). Existing approaches have notable limitations: (1) Dense visual prompting with VLMs can achieve strong performance but is costly in terms of both financial resources and carbon footprint, making it impractical for robotics applications. (2) Neuro-symbolic reasoning methods for 3D scene understanding fail to integrate visual inputs when synthesizing programs, making them ineffective in handling complex corner cases. To this end, we propose a fast-slow neuro-symbolic lane topology extraction algorithm, named Chameleon, which alternates between a fast system that directly reasons over detected instances using synthesized programs and a slow system that utilizes a VLM with a chain-of-thought design to handle corner cases. Chameleon leverages the strengths of both approaches, providing an affordable solution while maintaining high performance. We evaluate the method on the OpenLane-V2 dataset, showing consistent improvements across various baseline detectors. Our code, data, and models are publicly available at https://github.com/XR-Lee/neural-symbolic

==> tab4_ablation_speed.tex <==
\begin{table*}[ht]
\centering
\caption{Ablation Study of Model Components}
\begin{tabular}{ccc}
\toprule
\textbf{Method}  & \textbf{ TOP\_ll(AP\%)} &\textbf{ TOP\_lt(AP\%)} \\
\midrule
Prompt to symbolic     & xxx         & xxx \\
+ Expert Rule          & xxx         & xxx \\
+ Few-shot examples    & xxx         & xxx \\
+ VQA based reasoning  & xxx         & xxx\\
Full Model             & \textbf{xx} & xxx \\
\bottomrule
\end{tabular}
\label{tab:ablation_study}
\end{table*}

==> table5_ablation_lste.tex <==
\begin{table}[ht]
\centering
\caption{Ablation Study of Model Components}
\begin{tabular}{ccc}
\toprule
\textbf{Method}  & \textbf{ TOP\_lt(AP\%)}   \\
\midrule
Pair-wise Prompt to symbolic   & xxx         \\
+ Expert Rule                  & xxx        \\
+ Few-shot examples            & xxx           \\
+ VQA based reasoning          & xxx           \\
Full Model                     & \textbf{xx}   \\
        \bottomrule
    \end{tabular}
    \label{tab:ablation_study_lste}
    \vspace{-0.5cm}
\end{table}
